Bridging Information Security and Environmental Criminology Research to Better Mitigate Cybercrime

Cybercrime is a complex phenomenon that spans both technical and human aspects. As such, two disjoint areas have been studying the problem from separate angles: the information security community and the environmental criminology one. Despite the large body of work produced by these communities in the past years, the two research efforts have largely remained disjoint, with researchers on one side not benefitting from the advancements proposed by the other. In this paper, we argue that it would be beneficial for the information security community to look at the theories and systematic frameworks developed in environmental criminology to develop better mitigations against cybercrime. To this end, we provide an overview of the research from environmental criminology and how it has been applied to cybercrime. We then survey some of the research proposed in the information security domain, drawing explicit parallels between the proposed mitigations and environmental criminology theories, and presenting some examples of new mitigations against cybercrime. Finally, we discuss the concept of cyberplaces and propose a framework in order to define them. We discuss this as a potential research direction, taking into account both fields of research, in the hope of broadening interdisciplinary efforts in cybercrime research.

==> crime_patterns.tex <==
\subsection{Crime Patterns in Cyberspace}
\label{sec:crime_patterns}
Besides the similarity in the underlying crime principles in cyberspace versus the physical world, there is also considerable evidence of the presence of well-established crime patterns in cyberspace.

% Repeat/Near-repeat victimisation
%\subsubsection{Repeat and Near-Repeat Victimisation.}
\noindent \textbf{Repeat and Near-Repeat Victimisation.}
The phenomena of repeat and near-repeat victimisation (victims and their neighbours or close contacts experiencing a temporarily increased likelihood of being re-victimised) are highly proliferous in cybercrime.
Those who engage in cyberbullying and harassment are highly likely to harass the same individual or their close contacts over a period of time~\cite{henry_technology-facilitated_2018,reyns_situational_2010,tokunaga_following_2010}.
Due to the deceptive nature of the criminal market where e-mail, banking, and credit card credentials are illegally exchanged, the same information is often sold to (and thus, exploited by) multiple buyers in order to maximise profits~\cite{moore_nobody_2010}.
Onaolapo, Mariconti, and Stringhini~\cite{onaolapo_what_2016} identify that cybercriminals may access compromised accounts multiple times to steal more information, send spam messages, or use the account for further illicit activities.

Some forms of malware, such as the \emph{Code-Red}~\cite{moore_code-red:_2002} and \emph{Mabir}~\cite{bose_agent-based_2011} worms, tend to spread to nearby devices as much as possible.
Other forms of malware, such as the \emph{Zeus}~\cite{binsalleeh_analysis_2010}, \emph{Torpig}~\cite{stone2011analysis}, \emph{Pushdo/Cutwail}~\cite{stringhini_harvester_2014,stone-gross_underground_2011}, and other botnet malware families, tend to repeatedly use compromised devices to steal sensitive files and information, send spam messages, or carry out denial-of-service attacks.
Vulnerabilities in web page plugins (\eg Flash) expose users to repeated malvertisement-based attacks~\cite{zarras2014dark,sood_malvertising_2011,ford_analyzing_2009}.
Vasek, Wadleigh, and Moore~\cite{vasek_hacking_2016} and Vasek and Moore~\cite{vasek_identifying_2014} found that under 5\% of compromised WordPress websites are subsequently updated, while those that are not updated are re-compromised about twice as often as those that are.

% Crime Generators, Attractors, Enablers.
%\subsubsection{Crime Hotspots.}
\noindent \textbf{Crime Hotspots.}
There are three main types of crime hotspots in environmental criminology: \emph{crime generators}, \emph{crime attractors}, and \emph{crime enablers}.
As in the physical world, there are also instances of these types of hotspots occurring in the digital world.

Online marketplaces such as \emph{eBay}, \emph{Amazon}, and \emph{Gumtree} could be identified as crime generators in cyberspace -- places to which large numbers of people are attracted for reasons unrelated to crime.
Users browse these sites in order to purchase or sell products, but in doing so, they may become aware of peculiarities within each service that they may exploit, enabling criminal opportunities such as buyer fraud (\eg false item disputes in order to retain the purchased goods and recover one's money) or seller fraud (\eg sales of fake or illegal items).
Other examples of crime generators in cyberspace include online multiplayer or role-playing games, especially where minors and other vulnerable players abound, and their associated gaming forums.
In such ``cyber places'', some malicious players become aware of criminal opportunities to exploit other players, such as in online fraud (\eg falsely promising other gamers virtual goods or currency in exchange for real-world money), child sexual exploitation (\eg luring minors onto webcam-enabled services or real-world locations to perform sexual acts), or various other forms of cyberharassment and coercion.

In the digital world, there are certain services where cybercriminal activity is prominent and, quite frankly, to be expected. These are crime attractors -- places that are well known to offenders for their abundance in criminal opportunity.
Examples of such crime attractors include underground forums and marketplaces such as Silk Road, which was an infamous hub on the Dark Web for the trade of illegal products and services. Still on illegal trafficking, P2P software (\eg BitTorrent, Limewire), which are commonly used for the purposes of sharing illegal or explicit content, are also crime attractors, as such services are also common mechanisms for the discreet distribution of malware.

Certain software and websites exhibit crime attracting qualities too.
Roughly 80\% of the world's computer devices run a Windows operating system.
This corresponds to the majority of attacks being conducted against it, despite it having fewer vulnerabilities than other operating systems~\cite{noauthor_top_nodate}.
Web sites with certain characteristics, such as running the \emph{WordPress} or \emph{Joomla} CMSes, their traffic statistics, webpage structures, or the presence of certain keywords, are more likely to be hacked or subjected to predatory offending (spam, consumer fraud, \etc) than others~\cite{soska_automatically_2014}.
There is also a positive correlation between CMSes with the highest market share and the number of website compromises~\cite{vasek_hacking_2016,vasek_identifying_2014}.
Pirate websites (\eg illegal streaming services) are more likely to host malware~\cite{telang2018does}.
Vulnerable and/or deceptive browser extensions are commonly used to enable adware, spyware, and malvertisements~\cite{zarras2014dark,sood_malvertising_2011,ford_analyzing_2009} as well as being potential gateways for more serious malware infiltration~\cite{kotzias2016measuring,thomas2016investigating}.
Malware is increasingly being distributed on mobile devices through app stores, especially via illegitimate variants of Google Play and Apple AppStore.
Perhaps this is due to the apparent opportunity where access to official app stores are usually restricted for large populations in other parts of the world (\eg Asia)~\cite{ng2014android}.

Crime enablers -- places that facilitate crime due to the lack of place management or guardianship -- are also common analogous hotspots in cyberspace.
Social media sites, forums, and instant messengers are all ubiquitous services where cyberbullying, cyberstalking, and other forms of harassment take place.
Particularly with these services, most victims and offenders can easily gain access to them without any parental guardianship, while at the same time, the task of automatically detecting and blocking each instance of cyberharassment remains an ongoing challenge.
From an information security standpoint, websites and software with numerous or easily identifiable vulnerabilities are also examples of crime enablers.
For instance, websites that are not protected against (reasonably well known) SQL injection or cross-site scripting attacks could easily become compromised and used to commit further crimes, such as illegally accessing data stored on the server, or delivering malware to visiting users.
Also, besides software having unresolved and/or unmitigated vulnerabilities, devices and networks that lack any form of antivirus software or firewall protection, for example, are much more likely to be compromised by an attacker or malware instance than those that do not.
Previous research has shown that ISPs with poor security hygene ended up attracting malicious websites, since criminals felt that their operations would last longer if they were hosted on them~\cite{stone2009fire}.
Similarly, previous research has shown that criminals chose to heavily use banks with poor operational security to handle their fraudulent payments~\cite{levchenko_click_2011}.

